Quantifying and Improving the Accuracy of Electromagnetic Transient-Transient Stability Hybrid Simulation

The increasing penetration of inverter-based resources introduces new dynamic challenges to modern power grids, such as sub- and super-synchronous oscillations and other faster dynamics. These dynamics are typically fast in nature and are difficult to accurately model and analyze using standard transient stability (TS) methods, necessitating the need for electromagnetic transient (EMT) analysis. However, EMT simulations are notoriously slow for large-scale grids due to both equation formulations and computational limitations. To overcome this challenge, EMT-TS hybrid simulation is often used, since it offers a balanced trade-off between accuracy and speed, making it feasible to perform EMT analysis on large systems. One open question about EMT-TS hybrid simulation is the accuracy of the EMT-TS boundary or interface. This paper introduces an error index to quantify EMT-TS hybrid interface errors, identifies conditions where the hybrid simulation approach may become inaccurate, and suggests EMT region expansions to improve the simulation accuracy. Additionally, a three-sequence hybrid interface model is proposed to mitigate inaccuracies caused by unbalanced conditions.

==> app.tex <==
\appendix
{\color{red}
\section{Appendix A}
\label{sec:appA}

This appendix shows that the proposed error index in (\ref{eq:eidx}) has the same unit as the true error in (\ref{eq:etrue}) and their values have comparable magnitudes. 

Note that (\ref{eq:eidx}) and (\ref{eq:etrue}) differ only in their integrands. The integrand in (\ref{eq:etrue}) represents the per-unit voltage magnitude error, denoted as $\Delta V_{\text{m,pu}}(t)$, while the integrand in (\ref{eq:eidx}) contains the sum of squared errors in instantaneous three-phase voltage (in physical unit) between EMT side and TS side of the same bus. Assume that the errors in three phases are equal, then (\ref{eq:eidx_integrand}) becomes

\begin{equation}
	\Delta V_{\text{diff}} (t) = {\frac{\sqrt{3}}{\sqrt{6} V_{\text{B}}} \|V_{\text{a,h\_emt}} (t) - V_{\text{a,h\_ts}} (t)\|}.  \label{eq:app1}
\end{equation}

Suppose

\begin{subequations}
    \begin{eqnarray}
    \begin{aligned}
	    V_{\text{a,h\_emt}} (t) &= \sqrt{2} V_{\text{m,h\_emt,pu}}(t)\frac{V_{\text{B}}}{\sqrt{3}}\cos(2\pi f_0 t+\phi_{\text{emt}}(t))\label{eq:app2_1}\\
        V_{\text{a,h\_ts}} (t) &= \sqrt{2} V_{\text{m,h\_ts,pu}}(t)\frac{V_{\text{B}}}{\sqrt{3}}\cos(2\pi f_0 t+\phi_{\text{ts}}(t))\label{eq:app2_2}
        \end{aligned}
    \end{eqnarray}\label{eq:app2}
\end{subequations}

Then, assume

\begin{subequations}
    \begin{eqnarray}
    \begin{aligned}
        \phi_{\text{emt}}(t)&\approx\phi_{\text{ts}}(t)\\
        \|V_{\text{m,h\_emt,pu}}(t)-V_{\text{m,h\_ts,pu}}(t)\|&\approx \Delta V_{\text{m,pu}}(t)
        \end{aligned}
    \end{eqnarray}\label{eq:app3}
\end{subequations}

Then, (\ref{eq:app1}) becomes

% \Delta V_{\text{m}} = \frac{V_{\text{B}}}{\sqrt{3}}\Delta V_{\text{m,pu}}

\begin{equation}
\begin{aligned}
	\Delta V_{\text{diff}} (t) &\approx {\frac{\sqrt{3}}{\sqrt{6} V_{\text{B}}} \frac{\sqrt{2}V_{\text{B}}\Delta V_{\text{m,pu}}(t)}{\sqrt{3}} \|\cos(\omega t+\phi_{\text{ts}})\|}\\
    &= \Delta V_{\text{m,pu}}(t)\|\cos(\omega t+\phi_{\text{ts}})\|\\
    &\approx \frac{2}{\pi}\Delta V_{\text{m,pu}}(t).  \label{eq:app4}
    \end{aligned}
\end{equation}



}
